CaptainCook4D: A Dataset for Understanding Errors in Procedural Activities

Following step-by-step procedures is an essential component of various activities carried out by individuals in their daily lives. These procedures serve as a guiding framework that helps to achieve goals efficiently, whether it is assembling furniture or preparing a recipe. However, the complexity and duration of procedural activities inherently increase the likelihood of making errors. Understanding such procedural activities from a sequence of frames is a challenging task that demands an accurate interpretation of visual information and the ability to reason about the structure of the activity. To this end, we collect a new egocentric 4D dataset, CaptainCook4D, comprising 384 recordings (94.5 hours) of people performing recipes in real kitchen environments. This dataset consists of two distinct types of activity: one in which participants adhere to the provided recipe instructions and another in which they deviate and induce errors. We provide 5.3K step annotations and 10K fine-grained action annotations and benchmark the dataset for the following tasks: supervised error recognition, multistep localization, and procedure learning

==> paper_tex_files/table_tex_files/early_error_recognition.tex <==
\begin{wraptable}{r}{0.49\textwidth} 
    \centering
    \captionsetup{font=small}
    \caption{Early Error Recognition}
    \renewcommand{\arraystretch}{1.2} % Adjusts the row height
    \resizebox{0.45\textwidth}{!}{%
        \begin{tabular}{lcccc}
        \hline
        \textbf{Baseline}  & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} & \textbf{AUC Score} \\ \hline
        \textbf{3D ResNet} & 72.73              & 3.52            & 6.72              & 0.77               \\
        \textbf{Slowfast}  & 72.41              & 9.25            & 16.41             & 0.75               \\
        \textbf{X3D}       & 58.33              & 3.08            & 5.86              & 0.73               \\
        \textbf{VideoMAE}  & 70                 & 6.54            & 11.97             & 0.82               \\
        \textbf{Omnivore}  & 72.09              & 13.66           & 22.96             & 0.83               \\ \hline
        \end{tabular}%
    }
    \label{tab:ErrorEarlyPrediction}
\end{wraptable}

==> paper_tex_files/table_tex_files/error_category_recognition.tex <==
\begin{table*}[ht]
\captionsetup{font=small}
\caption{Error Category Recognition}
\label{tab:enhanced-error-detection}
\centering
\renewcommand{\arraystretch}{1.4} % Adjusts the row height
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccccccc}
\hline

\multicolumn{1}{c}{\textbf{Method Name}} &
\multicolumn{4}{c}{\textbf{Technique Error}} &
\multicolumn{4}{c}{\textbf{Preparation Error}} &
\multicolumn{4}{c}{\textbf{Measurement Error}} &
\multicolumn{4}{c}{\textbf{Temperature Error}} &
\multicolumn{4}{c}{\textbf{Timing Error}} \\

\cmidrule(lr){2-5}
\cmidrule(lr){6-9}
\cmidrule(lr){10-13}
\cmidrule(lr){14-17}
\cmidrule(lr){18-21}
  
&
  \textbf{Acc.} &
  \textbf{Prec.} &
  \textbf{Rec.} &
  \textbf{F1} &
  \textbf{Acc.} &
  \textbf{Prec.} &
  \textbf{Rec.} &
  \textbf{F1} &
  \textbf{Acc.} &
  \textbf{Prec.} &
  \textbf{Rec.} &
  \textbf{F1} &
  \textbf{Acc.} &
  \textbf{Prec.} &
  \textbf{Rec.} &
  \textbf{F1} &
  \textbf{Acc.} &
  \textbf{Prec.} &
  \textbf{Rec.} &
  \textbf{F1} \\
\hline
\textbf{3D ResNet} &
  88.56 & 27.91 & 18.18 & 22.02 &
  89.77 &  9.30 &  9.76 &  9.52 &
  88.43 &  6.98 &  6.12 &  6.52 &
  93.14 &  0.00 &  0.00 &  0.00 &
  91.52 &  6.98 & 11.54 &  8.70 \\
\textbf{Slowfast} &
  82.50 & 19.23 & 30.30 & 23.53 &
  83.45 & 10.58 & 26.83 & 15.17 &
  82.10 &  9.62 & 20.41 & 13.07 &
  85.20 &  0.96 & 12.50 &  1.79 &
  84.12 &  5.77 & 23.08 &  9.23 \\
\textbf{X3D} &
  83.31 &  9.72 & 10.61 & 10.14 &
  87.21 & 12.50 & 21.95 & 15.93 &
  85.33 &  8.33 & 12.24 &  9.92 &
  89.23 &  0.00 &  0.00 &  0.00 &
  87.62 &  4.17 & 11.54 &  6.12 \\
\textbf{VideoMAE} &
  84.39 & 19.18 & 22.22 & 20.59 &
  86.99 & 13.70 & 27.03 & 18.18 &
  84.39 &  8.22 & 12.77 & 10.00 &
  88.58 &  1.37 & 12.50 &  2.47 &
  87.14 &  6.85 & 19.23 & 10.10 \\
\textbf{Omnivore} &
  78.20 & 17.57 & 39.39 & 24.30 &
  80.22 & 14.19 & 51.22 & 22.22 &
  78.33 & 12.16 & 36.73 & 18.27 &
  79.81 &  2.03 & 37.50 &  3.85 &
   79.00 &  6.08 & 34.62 & 10.34 \\
\hline
\end{tabular}%
}
\end{table*}

==> paper_tex_files/table_tex_files/procedure_learning.tex <==
\begin{table}[!t]
\centering
\footnotesize
\captionsetup{font=small}
\caption{ \textbf{Procedure Learning.} Here, $\mathcal{P}$ represents precision, $R$ represents recall, and $I$ represents IOU.}
% \begin{tabular}{lcccccccccccc}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{
        l  % First column for Recipe names
        *{9}{r}  % 15 columns with fixed widths
    }
\toprule
\multirow{2}{*}{\textbf{Recipe}} & \multicolumn{3}{c}{Random} & \multicolumn{3}{c}{$\mathcal{M}_1$ \citep{dwibedi_et_al_2019}} \hline& \multicolumn{3}{c}{$\mathcal{M}_2$\citep{bansal_siddhant_my_2022}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
 & \CCOL{$\mathcal{P}$} & \CCOL{$\mathcal{R}$} & \CCOL{$\mathcal{I}$} & \CCOL{$\mathcal{P}$} & \CCOL{$\mathcal{R}$} & \CCOL{$\mathcal{I}$} & \CCOL{$\mathcal{P}$} & \CCOL{$\mathcal{R}$} & \CCOL{$\mathcal{I}$}   \\
\midrule
BlenderBananaPancakes       & 7.40          & 3.83          & 2.26          & 12.65          & 9.50           & 5.16          & 15.54          & 9.96           & 5.72          \\
Coffee                      & 6.54          & 3.87          & 2.17          & 13.68          & 9.91           & 5.49          & 15.76          & 10.25          & 5.63          \\
MugCake                     & 5.45          & 4.00          & 2.12          & 16.12          & 12.95          & 6.87          & 10.32          & 8.85           & 4.40          \\
PanFriedTofu                & 5.35          & 3.97          & 1.54          & 8.86           & 10.39          & 3.75          & 9.34           & 12.44          & 3.87          \\
Pinwheels                   & 6.54          & 4.28          & 2.13          & 13.58          & 11.96          & 5.92          & 16.08          & 13.06          & 7.05          \\ \midrule
\textbf{Average of 24 recipes}                   & \textbf{7.61} & \textbf{3.92} & \textbf{2.22} & \textbf{15.62} & \textbf{10.85} & \textbf{5.78} & \textbf{15.78} & \textbf{10.68} & \textbf{5.82} \\
\bottomrule
\end{tabular}
}
\vspace{-5mm}
\label{tab:ProcedureLearning}
\end{table}
